On rectangle-decomposable 2-parameter persistence modules

This paper addresses two questions: (a) can we identify a sensible class of 2-parameter persistence modules on which the rank invariant is complete? (b) can we determine efficiently whether a given 2-parameter persistence module belongs to this class? We provide positive answers to both questions, and our class of interest is that of rectangle-decomposable modules. Our contributions include: on the one hand, a proof that the rank invariant is complete on rectangle-decomposable modules, together with an inclusion-exclusion formula for counting the multiplicities of the summands; on the other hand, algorithms to check whether a module induced in homology by a bifiltration is rectangle-decomposable, and to decompose it in the affirmative, with a better complexity than state-of-the-art decomposition methods for general 2-parameter persistence modules. Our algorithms are backed up by a new structure theorem, whereby a 2-parameter persistence module is rectangle-decomposable if, and only if, its restrictions to squares are. This local characterization is key to the efficiency of our algorithms, and it generalizes previous conditions derived for the smaller class of block-decomposable modules. It also admits an algebraic formulation that turns out to be a weaker version of the one for block-decomposability. By contrast, we show that general interval-decomposability does not admit such a local characterization, even when locality is understood in a broad sense. Our analysis focuses on the case of modules indexed over finite grids, the more general cases are left as future work.

==> preliminaries.tex <==
% \label{sec:prelim}
% \paragraph{Product posets} Let $\abscisse$ and $\ordinates$ be subsets of $\R$ and consider the \emph{product poset} $X\times Y$ as the cartesian product $\poset$ equipped with the \emph{product order} $\leq$ defined by
% \begin{equation}
%     \forall s,t\in\poset,\, s \leq t \Longleftrightarrow s_x \leq t_x \text{ and } s_y \leq t_y,
% \end{equation}
% where the coordinates of a point $u\in\poset$ are denoted by $(u_x,u_y)$.
% We simply use the notation $\poset$ instead of $(\poset,\leq)$ as the only order considered on $\poset$ is the product order. 
% We say that a product poset is a \textit{finite grid} if $X$ and $Y$ are finite sets.
% \paragraph{Decomposability} We say that a persistence module over $U$ is \emph{decomposable} if it decomposes as the direct sum of two non-trivial persistence modules. Otherwise, we say that it is \emph{indecomposable}.
% Furthermore, two persistence modules are \emph{isomorphic} if they are naturally isomorphic as functors $\poset\to \cat{vec}$. 

% We also introduce a stronger notion of decomposability: if $\cat{C} = \{M_\alpha\}$ is a set of non-trivial indecomposable persistence modules $M_\alpha: \poset\to \cat{vec}$, then we say that persistence module $\basemod$ indexed over $U$ is \emph{$\cat{C}$-decomposable} if it decomposes as:
% \begin{equation*}
%     \basemod \cong \bigoplus_{\alpha\in A} \basemod_\alpha
% \end{equation*}
% where every $M_\alpha$ is a member of $\cat{C}$. 

% \paragraph{Interval, rectangle and block modules} Let $\perp$ be the binary relation defined by $s \perp t$ if, and only if $s \leq t$ or $t \leq s$. We say that a subset $Q$ of $\poset$ is \emph{path-connected} if for every $s,t$ in $\poset$, there exists a sequence of points $s = p_0 \perp \dots \perp p_n = t$. Furthermore, a subset $Q$ of $\poset$ is \emph{convex} if $t\in Q$ whenever $s\leq t \leq u$ and $s,u\in Q$. Now, we say that $Q\subseteq\poset$ is an \emph{interval} if it is convex and path-connected. 

%A rectangle $R$ of $\poset$ is a \emph{block} if $R = J_1 \times J_2$ with $J_1$ and $J_2$ being of at least one of the following forms: $J_i= (-\infty,a_i|$ with $a_i \in \R$ and the notation $|$ meaning that the interval can be open or closed on this end, or $J_i= |a_i,+\infty)$ with $a_i \in \R$, or $J_1= X$, or $J_2= Y$. 

% For an interval $Q$ of $\poset$, we define the \emph{indicator persistence module over $Q$} $\indimod[Q]$ by letting
% \begin{align*}
%    \field_{Q,t}=
%     \begin{cases}
%         \field &(t\in Q) \\
%         0 &(t\notin Q)
%     \end{cases} & & 
%       \indimod[Q](s\leq t) =
%     \begin{cases}
%         \identity_\field &\mbox{ if } s \mbox{ and } t \in Q, \\
%         0 &\mbox{ else}.
%     \end{cases}
% \end{align*}

% By convention, we set $\indimod[\emptyset]= \zeromod$. We define a persistence module over $(\poset,\leq)$ to be a \emph{interval module} if it is the indicator module of an interval.
% We define \emph{rectangle modules} and \emph{block modules} similarly.
%  let $\cat{Int}$ denote the set of interval modules in $\poset$. 

%We define a persistence module over $(\poset,\leq)$ to be a \emph{block module} if it is the indicator module of a block, and we denote $\cat{Blc}(\poset,\leq)$ the full subcategory of $\cat{Per}$ with objects the block modules. When there is no room for confusion, we simply denote by $\cat{Blc}$ this category.

%\subsection{Decomposability results}
%A persistence module $M$ is pointwise finite-dimensional (pfd) if $\dim M_p < \infty $ for all $p\in \poset$.

% \begin{thm}[\cite{botnan2018decomposition}]
% Any pointwise finite-dimensional persistence module is a direct sum of indecomposable modules with local endomorphism ring\footnote{A technical condition which ensures that such a direct sum decomposition is essentially unique; see \cite{Azumaya1950}.}
% \end{thm}
% We remark that the previous theorem has a particularly simple inductive proof when $\poset$ is a finite grid. 

% The following theorem is fundamental to topological data analysis. The case where $U=\libr 1, n\ribr$ will be instrumental in the proof of our main result. 

% \begin{thm}\label{thm:1D}
% Any pointwise-finite dimensional persistence module $M\colon U\subseteq \R \to \cat{vec}$ decomposes into a direct sum of interval modules.
% \end{thm}

%Moving beyond single-parameter persistence we observed in the introduction that decompositions in general are more complicated. The following result is well-known, see for instance Theorem 3 and Figure 13 in \cite{Escolar_2015}.
%
%\begin{prop}
%Let $S = \{a,b,c,d\}$ denote the corners of a rectangle in $\R^2$. Any pointwise-finite dimensional persistence module $M\colon S\to \cat{vec}$ is interval-decomposable. 
%\end{prop}
%The set of intervals $\mathcal{I}$ in $S$ is
%\begin{equation}
%    \mathcal{I}=\{\{\{a\},\{d\},\{a,b\},\{a,c\},\{b,d\},\{c,d\},\{a,b,c\},\{b,c,d\},\{a,b,c,d\}\}, 
%\end{equation}
%The subset $\mathcal{B}\subseteq\mathcal{I}$ of blocks of $S$ is
%\begin{equation}
%    \mathcal{B} = \{\{a\},\{d\},\{a,b\},\{a,c\},\{b,d\},\{c,d\},\{a,b,c,d\}\}.
%\end{equation} 
%If $\mathcal{C}\subseteq\mathcal{I}$, an element of $\mathcal{C}$ is called a $\mathcal{C}$-interval.
% We say that a persistence module indexed by $S$ is $\mathcal{B}$-decomposable if it decomposes into interval modules supported on intervals in $\mathcal{B}$. 

%In \cite{Cochoy2016}, Cochoy and Oudot introduced the notion of \emph{strongly exact modules} and showed that such modules decompose into a particular class of rectangle modules called \emph{blocks}. The algebraic formulation of strongly exact will be stated below, but an equivalent formulation at the geometric level is as follows: a persistence module $M$ is strongly exact if its restriction to any square $S$ in its support is $\mathcal{B}$-decomposable. Interestingly, this shows that for a certain class of modules the global structure can be inferred from local geometric properties. A slightly more general formulation of the following can be found in \cite{botnan2018decomposition}. 
%
%\begin{thm}\textnormal{\cite[Thm.~2.1]{Cochoy2016}}
%    A pfd persistence module indexed over $\poset$ is block-decomposable if, and only if, its restriction to any square is block-decomposable.
%\end{thm} 

% A persistence bimodule $\basemod$ over $(\poset,\leq)$ is said to be \emph{strongly exact} if for all $s\leq t\in \poset$, the following sequence is exact:
% \begin{equation*}
%     M_s \xrightarrow{\mor_s^{(t_x,s_y)}\oplus \mor_s^{(s_x,t_y)}} M_{(s_x,t_y)}\oplus M_{(t_x,s_y)} \xrightarrow{\mor_{(s_x,t_y)}^t - \mor_{(t_x,s_y)}^t} M_t.
% \end{equation*}

%\begin{que}[Main question]
%    \label{que:main}
%    What choice of full subcategory $\cat{C}\subseteq\cat{Int}$ gives, for any persistence bimodule, an equivalence between its $\cat{C}$-decomposability and the $\cat{C}$-decomposability of its restriction to any square?
%    \todo{Put Persistence}
%\end{que}

%Define $a=(0,0)$, $b=(0,1)$, $c=(1,0)$ and $d=(1,1)$, and consider the square $(S,\leq)$, where $S = \{a,b,c,d\}$, and $\leq$ is the product order. This poset can be represented by the diagram:
%\begin{equation*}
%    \begin{tikzcd}
%        b \arrow[r]           & d           \\
%        a \arrow[r] \arrow[u] & c \arrow[u]
%    \end{tikzcd}
%\end{equation*}
%Since any square is canonically isomorphic as a poset to $(S,\leq)$, a persistence module over any square can be seen as a persistence module over $(S,\leq)$. We can then always consider restrictions of persistence bimodule to squares as persistence modules over $(S,\leq)$, and focus on persistence modules over $(S,\leq)$ to study the decomposability of the restrictions. The set $\mathcal{I}$ of intervals of $(S,\leq)$ is
%
%
%It is well known that (\todo{Ref or prove}) a persistence module over a square is always $\cat{Int}$-decomposable. Remarkably, the result of Cochoy and Oudot\cite{Cochoy2016} states that a pfd persistence bimodule is $\cat{Blc}$-decomposable if, and only if, its restrictions to any square contains only $\mathcal{B}$-intervals in their decomposition into interval summands. One may then naturally wonder what additional intervals can one add to the collection $\mathcal{B}$ so that the equivalence of decomposability still holds. 
%
%The first result of this article proves that if one adds the intervals $\{b\}$ and $\{c\}$ to the collection $\mathcal{B}$, obtaining the set $\mathcal{R}$ of rectangles of $(S,\leq)$, the equivalence still holds when $\poset$ is a finite grid, as stated by the next theorem.
%Moreover, the rectangle-decomposability of persistence modules over squares is fully characterized by an algebraic condition called weak exactness (see \Cref{def:weak-exactness}). As the name of this condition suggests, any strongly exact bimodule is weakly exact, but the converse is not true. This is coherent with the fact that any block-decomposable bimodule is rectangle-decomposable, but the converse is not true.
%
%The second result of this article proves that if one adds any remaining interval of the square, namely $\{a,b,c\}$ or $\{b,c,d\}$, then the equivalence of decomposability in \Cref{main:rec-dec} fails:
%\begin{prop}
%  The persistence module defined in \Cref{ex:3-2-indecomposable} is indecomposable and all its restriction to squares are decomposable into direct sums of interval modules supported on intervals of the set $\mathcal{R}\cup\{b,c,d\}$.
%\end{prop}
%Indeed, the persistence module of \Cref{ex:3-2-indecomposable} is indecomposable as we said previously, but it is not an interval module, as it is already not an indicator module. 


